Post-Quantum Hybrid Digital Signatures with Hardware-Support for Digital Twins

Digital Twins (DT) virtually model cyber-physical objects using Internet of Things (IoT) components (e.g., sensors) to gather and process senstive information stored in the cloud. Trustworthiness of the streamed data is crucial which requires quantum safety and breach resiliency. Digital signatures are essential for scalable authentication and non-repudiation. Yet, NIST PQC signature standards are exorbitantly costly for low-end IoT without considering forward security. Moreover, Post-Quantum (PQ) signatures lack aggregation, which is highly desirable to reduce the transmission and storage burdens in DTs. Hence, there is an urgent need for lightweight digital signatures that offer compromise resiliency and compactness while permitting an effective transition into the PQ era for DTs. We create a series of highly lightweight digital signatures called Hardware-ASsisted Efficient Signature (HASES) that meets the above requirements. The core of HASES is a hardware-assisted cryptographic commitment construct oracle (CCO) that permits verifiers to obtain expensive commitments without signer interaction. We created three HASES schemes: PQ-HASES is a forward-secure PQ signature, LA-HASES is an efficient aggregate Elliptic-Curve signature, and HY-HASES is a novel hybrid scheme that combines PQ-HASES and LA-HASES with novel strong nesting and sequential aggregation. HASES does not require a secure-hardware on the signer. We proved that HASES schemes are secure and implemented them on commodity hardware and an 8-bit AVR ATmega2560. Our experiments confirm that PQ-HASES and LA-HASES are two magnitudes of times more signer efficient than their PQ and conventional-secure counterparts, respectively. HY-HASES outperforms NIST PQC and conventional signature combinations, offering a standardcompliant transitional solution for emerging DTs. We open-source HASES schemes for public testing and adaptation.

==> relatedwork.tex <==
%\section{Related Work} \label{sec:RelatedWorkScope}
%We now briefly discuss related work that is complementary to ours or out of our scope. 
%
%{\em Aggregate Signatures for Audit Logging with Extended Properties}: The Forward-secure and Aggregate Signatures (FAS)~\cite{FssAggNew,Yavuz:2012:TISSEC:FIBAF,LogFASFC2012,SecureLogAttacks:2017:Hartung,Yavuz:CORE:CNS:2020,FAS_Asymptotic}) offer breach-resiliency and (partial) signature aggregation at the same time. Hence, they have been extensively studied in the context of secure audit logs. Despite their merits, FAS schemes introduce significant computation and storage overhead either at the signer and/or verifier sides. In our performance analysis, among all FAS alternatives, we selected FI-BAF~\cite{Yavuz:2012:TISSEC:FIBAF} as our main counterpart, since it is the most signer-efficient FAS. All other FAS schemes introduce significantly higher signer overhead along with expensive signature verification. Therefore, \opas~schemes are much more efficient than all these alternatives but without forward-security. 
%
%There is a line of work that offers advanced features for aggregate signatures such as fault tolerance (e.g., \cite{Aggregate:Sig:FaultToelrant:2018,AggregateFaulthTolerant:2021:Journal}), verifiable excerpts~\cite{Logging_VerifiableExcerpt}, and others~\cite{SecureLogHartungThesis2020}. They are complementary to our schemes. 
%
%
%{\em Other Related Work}:   There is a vast body of literature that aims to cope with the privacy issues in audit log systems. They harness various  Privacy Enhancing Technologies (PETs) such as searchable encryption~\cite{SecureLogPairingSearchable,davis2004time,shi2007multi,zhao2018privacy} and others~\cite{ramzan2022secure}. Another line of work focuses on Proof of Retrievability (PoR)~\cite{anthoine2021dynamic,shi2013practical,li2013efficient} on the outsourced client data. Finally, several works concentrate on the system and scalability of aspects of secure audit logs (e.g.,~\cite{hassan2020omegalog,liu2022transparent,yagemann2021validating}). Some of these works can be complementary to ours.  
